Horizon-Free Reinforcement Learning in Polynomial Time: the Power of Stationary Policies

This paper gives the first polynomial-time algorithm for tabular Markov Decision Processes (MDP) that enjoys a regret bound \emph{independent on the planning horizon}. Specifically, we consider tabular MDP with $S$ states, $A$ actions, a planning horizon $H$, total reward bounded by $1$, and the agent plays for $K$ episodes. We design an algorithm that achieves an $O\left(\mathrm{poly}(S,A,\log K)\sqrt{K}\right)$ regret in contrast to existing bounds which either has an additional $\mathrm{polylog}(H)$ dependency~\citep{zhang2020reinforcement} or has an exponential dependency on $S$~\citep{li2021settling}. Our result relies on a sequence of new structural lemmas establishing the approximation power, stability, and concentration property of stationary policies, which can have applications in other problems related to Markov chains.

==> header.tex <==
\usepackage{bbm}
\usepackage{nicefrac}       % compact symbols for 1/2, etc.

\usepackage{amsmath,amsfonts,bm}
\usepackage{amssymb,amsthm}
\usepackage{mathtools}
\usepackage{algorithm,algorithmic}
\usepackage{appendix}
\usepackage{enumerate}

% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}

%\newtheorem{lemma}{Lemma}
%\newtheorem{corollary}{Corollary}
%\newtheorem{theorem}{Theorem}
%\newtheorem{assumption}{Assumption}
%\newtheorem{definition}{Definition}
%\newtheorem{proposition}{Proposition}
%\newtheorem{condition}{Condition}
%%\newtheorem{remark}{Remark}


\usepackage{enumerate}
\usepackage{enumitem}
%\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{mathtools}
%\mathtoolsset{showonlyrefs}
%\usepackage{booktabs}       % professional-quality tables
\usepackage{array}

\usepackage{footnote}
\usepackage{wrapfig}
\usepackage{graphicx}

\usepackage{pifont}
\newcommand{\xmark}{\text{\ding{55}}}
\newcommand{\cmark}{\text{\ding{51}}}
\usepackage{hhline}
\usepackage{makecell}


%for convenience
% \newenvironment{itemize*}%
% {\begin{itemize}[leftmargin=*,topsep=0pt]%
% 		\setlength{\itemsep}{0pt}%
% 		\setlength{\parskip}{0pt}}%
% 	{\end{itemize}}

% \newenvironment{enumerate*}%
% {\begin{enumerate}[leftmargin=*,topsep=0pt]%
% 		\setlength{\itemsep}{0pt}%
% 		\setlength{\parskip}{0pt}}%
% 	{\end{enumerate}}

%comments
\def\shownotes{0} 
\ifnum\shownotes=1
\newcommand{\simon}[1]{[\textcolor{red}{Simon: #1}]}
\newcommand{\zihan}[1]{\textcolor{red}{[Zihan: #1]}}

\else
\newcommand{\simon}[1]{}
\newcommand{\zihan}[1]{}

\fi


